Dense Subgraph Discovery Meets Strong Triadic Closure

Finding dense subgraphs is a core problem with numerous graph mining applications such as community detection in social networks and anomaly detection. However, in many real-world networks connections are not equal. One way to label edges as either strong or weak is to use strong triadic closure~(STC). Here, if one node connects strongly with two other nodes, then those two nodes should be connected at least with a weak edge. STC-labelings are not unique and finding the maximum number of strong edges is NP-hard. In this paper, we apply STC to dense subgraph discovery. More formally, our score for a given subgraph is the ratio between the sum of the number of strong edges and weak edges, weighted by a user parameter $\lambda$, and the number of nodes of the subgraph. Our goal is to find a subgraph and an STC-labeling maximizing the score. We show that for $\lambda = 1$, our problem is equivalent to finding the densest subgraph, while for $\lambda = 0$, our problem is equivalent to finding the largest clique, making our problem NP-hard. We propose an exact algorithm based on integer linear programming and four practical polynomial-time heuristics. We present an extensive experimental study that shows that our algorithms can find the ground truth in synthetic datasets and run efficiently in real-world datasets.

==> case-study/all-rows.tex <==

\begin{figure}
\begin{center}

\begin{tabular}{lll}


\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-1-a}
\node[anchor=south west] at (-0.5, -3) {(a)};
\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-1-b}
\node[anchor=south west] at (-0.5, -3) {(b)};
\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-1-c}
\node[anchor=south west] at (-0.5, -3) {(c)};
\end{tikzpicture}\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%2nd-row


\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-2-d}
\node[anchor=south west] at (-0.5, -3) {(d)};
\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-2-e}
\node[anchor=south west] at (-0.5, -3) {(e)};
\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-2-f}
\node[anchor=south west] at (-0.5, -3) {(f)};
\end{tikzpicture}\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%3rd-row

\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-3-g}
\node[anchor=south west] at (-0.5, -3) {(g)};
\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-3-h}
\node[anchor=south west] at (-0.5, -3) {(h)};
\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[scale = .75]
\tikzstyle{lm1} = [fill = yafcolor3!50!black, inner sep = 1.2pt]
\tikzstyle{lm2} = [circle, fill = yafcolor4!50!black, inner sep = 1pt]
\tikzstyle{lm3} = [circle, fill = gray!50, inner sep = 1pt]
\tikzstyle{ll} = []
%\tikzstyle{le1} = [yafcolor2, thick, bend left = 10, opacity = 0.5]
%\tikzstyle{le2} = [gray, bend left = 10, opacity = 0.5]
\tikzstyle{le1} = [yafcolor4, thick, bend left = 10]
\tikzstyle{le2} = [yafcolor5, thick, bend left = 10]
\tikzstyle{le3} = [gray!50, bend left = 10]
\input{case-study/r-3-i}
\node[anchor=south west] at (-0.5, -3) {(i)};
\end{tikzpicture}


\end{tabular}









\caption{
Strong~(Red) and weak~(Blue) edges of the \dtname{Karate}  dataset discovered by the algorithms  \alggreedyfastest, \algdenseg, and \algdensec in their respective order. Each row represents a specific of $\lambda$; $\lambda = 0.4, 0.6$, and $0.8$ respectively.
}
\label{fig:case-study}
\end{center}
\end{figure}


==> case-study/r-1-a.tex <==
% {0, 1, 2, 3, 7, 8, 13, 17, 18, 19, 20, 21, 23, 24, 25, 27, 30, 31, 32, 33}
\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm2] (n17) at (-1.278, -0.60231) {};
\node[lm2] (n18) at (0.51654, 1.9636) {};
\node[lm2] (n19) at (-0.30691, 0.035621) {};
\node[lm2] (n20) at (0.10109, 1.891) {};
\node[lm2] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm2] (n23) at (-0.2767, 1.6423) {};
\node[lm2] (n24) at (-1.5541, 0.77017) {};
\node[lm2] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm2] (n27) at (-0.5343, 0.9102) {};
\node[lm3] (n28) at (-0.16321, 0.83704) {};
\node[lm3] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm2] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};
% [(0, 1), (1, 2), (1, 3), (2, 3), (2, 7), (8, 30), (32, 33)]
% le1 strong le2 weak le3 grey
\begin{pgfonlayer}{background}
\draw (n0) edge[le1] (n1);
\draw (n1) edge[le1] (n2);
\draw (n1) edge[le1] (n3);
\draw (n2) edge[le1] (n3);
\draw (n2) edge[le1] (n7);
\draw (n8) edge[le1] (n30);
\draw (n32) edge[le1] (n33);


 % [(0, 2), (0, 3), (0, 7), (0, 8), (0, 13), (0, 17), (0, 19), (0, 21), (0, 31), (1, 7), (1, 13), (1, 17), (1, 19), (1, 21), (1, 30), (2, 8), (2, 13), (2, 27), (2, 32), (3, 7), (3, 13), (8, 32), (8, 33), (13, 33), (18, 32), (18, 33), (19, 33), (20, 32), (20, 33), (23, 25), (23, 27), (23, 32), (23, 33), (24, 25), (24, 27), (24, 31), (25, 31), (27, 33), (30, 32), (30, 33), (31, 32), (31, 33)]
\draw (n0) edge[le2] (n2);
\draw (n0) edge[le2] (n3);
\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le2] (n17);
\draw (n0) edge[le2] (n19);
\draw (n0) edge[le2] (n21);
\draw (n0) edge[le2] (n31);
\draw (n1) edge[le2] (n7);
\draw (n1) edge[le2] (n13);
\draw (n1) edge[le2] (n17);
\draw (n1) edge[le2] (n19);
\draw (n1) edge[le2] (n21);
\draw (n1) edge[le2] (n30);

\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le2] (n27);
\draw (n2) edge[le3] (n28);
\draw (n2) edge[le2] (n32);
\draw (n3) edge[le2] (n7);
\draw (n3) edge[le3] (n12);
\draw (n3) edge[le2] (n13);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);

\draw (n8) edge[le2] (n32);
\draw (n8) edge[le2] (n33);
\draw (n9) edge[le3] (n33);
\draw (n13) edge[le2] (n33);
\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le2] (n32);
\draw (n18) edge[le2] (n33);
\draw (n19) edge[le2] (n33);
\draw (n20) edge[le2] (n32);
\draw (n20) edge[le2] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);
\draw (n23) edge[le2] (n25);
\draw (n23) edge[le2] (n27);
\draw (n23) edge[le3] (n29);
\draw (n23) edge[le2] (n32);
\draw (n23) edge[le2] (n33);
\draw (n24) edge[le2] (n25);
\draw (n24) edge[le2] (n27);
\draw (n24) edge[le2] (n31);
\draw (n25) edge[le2] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le2] (n33);
\draw (n28) edge[le3] (n31);
\draw (n28) edge[le3] (n33);
\draw (n29) edge[le3] (n32);
\draw (n29) edge[le3] (n33);
\draw (n30) edge[le2] (n32);
\draw (n30) edge[le2] (n33);
\draw (n31) edge[le2] (n32);
\draw (n31) edge[le2] (n33);

\end{pgfonlayer}


% (0, 1), (0, 2), (0, 3), (0, 13), (1, 2), (1, 3), (1, 13), (2, 3), (2, 13), (3, 13)

% strong weak 7 42
%  len: 42 7  set: [(0, 2), (0, 3), (0, 7), (0, 8), (0, 13), (0, 17), (0, 19), (0, 21), (0, 31), (1, 7), (1, 13), (1, 17), (1, 19), (1, 21), (1, 30), (2, 8), (2, 13), (2, 27), (2, 32), (3, 7), (3, 13), (8, 32), (8, 33), (13, 33), (18, 32), (18, 33), (19, 33), (20, 32), (20, 33), (23, 25), (23, 27), (23, 32), (23, 33), (24, 25), (24, 27), (24, 31), (25, 31), (27, 33), (30, 32), (30, 33), (31, 32), (31, 33)] - [(0, 1), (1, 2), (1, 3), (2, 3), (2, 7), (8, 30), (32, 33)]
% lam: 0.4 density : 1.19 size: 20
% --- 0.14917421340942383 seconds ---
% {0, 1, 2, 3, 7, 8, 13, 17, 18, 19, 20, 21, 23, 24, 25, 27, 30, 31, 32, 33}




% V(W): 78  E(W): 393
% V(W): 29  E(W): 51
% charikar strong weak 8 22
%  len: 22 8  set: [(0, 2), (0, 7), (0, 8), (0, 13), (1, 2), (1, 7), (1, 13), (1, 30), (2, 7), (2, 8), (2, 13), (2, 32), (3, 13), (8, 30), (8, 32), (8, 33), (13, 33), (23, 32), (29, 32), (29, 33), (30, 32), (30, 33)] - [(0, 1), (0, 3), (1, 3), (2, 3), (3, 7), (23, 29), (23, 33), (32, 33)]
% charikar: lam: 0.4 density : 1.4000000000000001 size: 12
% --- 0.10455608367919922 seconds ---
% [0, 1, 2, 3, 7, 8, 13, 23, 29, 30, 32, 33]



% V(W): 78  E(W): 393
% V(W): 35  E(W): 76
% Goldberg  based: strong weak 9 26
%  len: 26 9  set: [(0, 1), (0, 7), (0, 8), (0, 13), (0, 31), (1, 2), (1, 7), (1, 30), (2, 7), (2, 8), (2, 13), (2, 32), (3, 7), (3, 13), (32, 8), (32, 23), (32, 29), (32, 30), (33, 13), (33, 23), (33, 29), (33, 30), (33, 31), (8, 30), (23, 25), (25, 31)] - [(0, 2), (0, 3), (1, 3), (1, 13), (2, 3), (32, 31), (32, 33), (33, 8), (23, 29)]
% goldberg: lam: 0.4 density : 1.3857142857142857 size: 14
% --- 0.2758636474609375 seconds ---
% [0, 1, 2, 3, 32, 33, 7, 8, 13, 23, 25, 29, 30, 31]

==> case-study/r-1-b.tex <==
% [0, 1, 2, 3, 32, 33, 7, 8, 13, 23, 25, 29, 30, 31]
\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm3] (n17) at (-1.278, -0.60231) {};
\node[lm3] (n18) at (0.51654, 1.9636) {};
\node[lm3] (n19) at (-0.30691, 0.035621) {};
\node[lm3] (n20) at (0.10109, 1.891) {};
\node[lm3] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm2] (n23) at (-0.2767, 1.6423) {};
\node[lm3] (n24) at (-1.5541, 0.77017) {};
\node[lm2] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm3] (n27) at (-0.5343, 0.9102) {};
\node[lm3] (n28) at (-0.16321, 0.83704) {};
\node[lm2] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm2] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};
% [(0, 2), (0, 3), (1, 3), (1, 13), (2, 3), (32, 31), (32, 33), (33, 8), (23, 29)]
\begin{pgfonlayer}{background}

\draw (n0) edge[le1] (n2);
\draw (n0) edge[le1] (n3);
\draw (n1) edge[le1] (n3);
\draw (n1) edge[le1] (n13);
\draw (n2) edge[le1] (n3);
\draw (n8) edge[le1] (n33);
\draw (n23) edge[le1] (n29);
\draw (n31) edge[le1] (n32);
\draw (n32) edge[le1] (n33);


% [(0, 1), (0, 7), (0, 8), (0, 13), (0, 31), (1, 2), (1, 7), (1, 30), (2, 7), (2, 8), (2, 13), (2, 32), (3, 7), (3, 13), (32, 8), (32, 23), (32, 29), (32, 30), (33, 13), (33, 23), (33, 29), (33, 30), (33, 31), (8, 30), (23, 25), (25, 31)] 
\draw (n0) edge[le2] (n1);
\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le3] (n17);
\draw (n0) edge[le3] (n19);
\draw (n0) edge[le3] (n21);
\draw (n0) edge[le2] (n31);
\draw (n1) edge[le2] (n2);
\draw (n1) edge[le2] (n7);
\draw (n1) edge[le3] (n17);
\draw (n1) edge[le3] (n19);
\draw (n1) edge[le3] (n21);
\draw (n1) edge[le2] (n30);
\draw (n2) edge[le2] (n7);
\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le3] (n27);
\draw (n2) edge[le3] (n28);
\draw (n2) edge[le2] (n32);
\draw (n3) edge[le2] (n7);
\draw (n3) edge[le3] (n12);
\draw (n3) edge[le2] (n13);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);
\draw (n8) edge[le2] (n30);
\draw (n8) edge[le2] (n32);

\draw (n9) edge[le3] (n33);
\draw (n13) edge[le2] (n33);
\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le3] (n32);
\draw (n18) edge[le3] (n33);
\draw (n19) edge[le3] (n33);
\draw (n20) edge[le3] (n32);
\draw (n20) edge[le3] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);
\draw (n23) edge[le2] (n25);
\draw (n23) edge[le3] (n27);

\draw (n23) edge[le2] (n32);
\draw (n23) edge[le2] (n33);
\draw (n24) edge[le3] (n25);
\draw (n24) edge[le3] (n27);
\draw (n24) edge[le3] (n31);
\draw (n25) edge[le2] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le3] (n33);
\draw (n28) edge[le3] (n31);
\draw (n28) edge[le3] (n33);
\draw (n29) edge[le2] (n32);
\draw (n29) edge[le2] (n33);
\draw (n30) edge[le2] (n32);
\draw (n30) edge[le2] (n33);
\draw (n31) edge[le2] (n33);
\end{pgfonlayer}


% (0, 1), (0, 2), (0, 3), (0, 13), (1, 2), (1, 3), (1, 13), (2, 3), (2, 13), (3, 13)

==> case-study/r-1-c.tex <==
% [0, 1, 2, 3, 7, 8, 13, 23, 29, 30, 32, 33]
\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm3] (n17) at (-1.278, -0.60231) {};
\node[lm3] (n18) at (0.51654, 1.9636) {};
\node[lm3] (n19) at (-0.30691, 0.035621) {};
\node[lm3] (n20) at (0.10109, 1.891) {};
\node[lm3] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm2] (n23) at (-0.2767, 1.6423) {};
\node[lm3] (n24) at (-1.5541, 0.77017) {};
\node[lm3] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm3] (n27) at (-0.5343, 0.9102) {};
\node[lm3] (n28) at (-0.16321, 0.83704) {};
\node[lm2] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm3] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};
\begin{pgfonlayer}{background}

 % [(0, 1), (0, 3), (1, 3), (2, 3), (3, 7), (23, 29), (23, 33), (32, 33)]
% strong

\draw (n0) edge[le1] (n1);
\draw (n0) edge[le1] (n3);
\draw (n1) edge[le1] (n3);
\draw (n2) edge[le1] (n3);
\draw (n3) edge[le1] (n7);
\draw (n23) edge[le1] (n29);
\draw (n23) edge[le1] (n33);
\draw (n32) edge[le1] (n33);





% [(0, 2), (0, 7), (0, 8), (0, 13), (1, 2), (1, 7), (1, 13), (1, 30), (2, 7), (2, 8), (2, 13), (2, 32), (3, 13), (8, 30), (8, 32), (8, 33), (13, 33), (23, 32), (29, 32), (29, 33), (30, 32), (30, 33)] 
% weak
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n1) edge[le2] (n7);
\draw (n1) edge[le2] (n30);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le2] (n32);
\draw (n3) edge[le2] (n13);
\draw (n13) edge[le2] (n33);


\draw (n0) edge[le2] (n2);
\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le3] (n17);
\draw (n0) edge[le3] (n19);
\draw (n0) edge[le3] (n21);
\draw (n0) edge[le3] (n31);
\draw (n1) edge[le2] (n2);
\draw (n1) edge[le2] (n13);
\draw (n1) edge[le3] (n17);
\draw (n1) edge[le3] (n19);
\draw (n1) edge[le3] (n21);
\draw (n2) edge[le2] (n7);
\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le3] (n27);
\draw (n2) edge[le3] (n28);
\draw (n3) edge[le3] (n12);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);
\draw (n8) edge[le2] (n32);
\draw (n8) edge[le2] (n30);
\draw (n8) edge[le2] (n33);
\draw (n9) edge[le3] (n33);

\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le3] (n32);
\draw (n18) edge[le3] (n33);
\draw (n19) edge[le3] (n33);
\draw (n20) edge[le3] (n32);
\draw (n20) edge[le3] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);
\draw (n23) edge[le3] (n25);
\draw (n23) edge[le3] (n27);

\draw (n23) edge[le2] (n32);

\draw (n24) edge[le3] (n25);
\draw (n24) edge[le3] (n27);
\draw (n24) edge[le3] (n31);
\draw (n25) edge[le3] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le3] (n33);
\draw (n28) edge[le3] (n31);
\draw (n28) edge[le3] (n33);
\draw (n29) edge[le2] (n32);
\draw (n29) edge[le2] (n33);
\draw (n30) edge[le2] (n33);
\draw (n30) edge[le2] (n32);
\draw (n31) edge[le3] (n32);
\draw (n31) edge[le3] (n33);

\end{pgfonlayer}

% strong

% (0, 1), (0, 2), (0, 3),  (0, 13), (1, 2), (1, 3), , (1, 13), (2, 3),, (2, 13),, (3, 13)

% weak
% (1, 7)
% (0, 7)
% (2, 7)
% (3, 7)


% strong
% (0, 1), (0, 2), (0, 3),  (0, 13), (1, 2), (1, 3), , (1, 13), , (2, 3), (2, 7), ,  (3, 7),  (32, 8), (32, 30), (32, 33), (33, 8),, (33, 30), (8, 30)


% Weak: 9 edges
% (0, 7)
% (1, 7)
% (3, 13),
% (2, 13)
% (1, 30)
%  (33, 13)
% (2, 8)
%  (2, 32)
%  (0, 8)


==> case-study/r-2-d.tex <==
% {0, 1, 2, 3, 7, 8, 13, 19, 20, 23, 24, 25, 27, 28, 29, 30, 31, 32, 33}
\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm3] (n17) at (-1.278, -0.60231) {};
\node[lm3] (n18) at (0.51654, 1.9636) {};
\node[lm2] (n19) at (-0.30691, 0.035621) {};
\node[lm2] (n20) at (0.10109, 1.891) {};
\node[lm3] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm2] (n23) at (-0.2767, 1.6423) {};
\node[lm2] (n24) at (-1.5541, 0.77017) {};
\node[lm2] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm2] (n27) at (-0.5343, 0.9102) {};
\node[lm2] (n28) at (-0.16321, 0.83704) {};
\node[lm2] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm2] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};
\begin{pgfonlayer}{background}


\draw (n0) edge[le1] (n1);
\draw (n0) edge[le1] (n2);
\draw (n0) edge[le1] (n3);
\draw (n1) edge[le1] (n2);
\draw (n2) edge[le1] (n3);
\draw (n1) edge[le1] (n7);
\draw (n8) edge[le1] (n30);
\draw (n23) edge[le1] (n29);
\draw (n23) edge[le1] (n33);
\draw (n24) edge[le1] (n31);
\draw (n32) edge[le1] (n33);




\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le3] (n17);
\draw (n0) edge[le2] (n19);
\draw (n0) edge[le3] (n21);
\draw (n0) edge[le2] (n31);
\draw (n1) edge[le2] (n3);
\draw (n1) edge[le2] (n13);
\draw (n1) edge[le3] (n17);
\draw (n1) edge[le2] (n19);
\draw (n1) edge[le3] (n21);
\draw (n1) edge[le2] (n30);
\draw (n2) edge[le2] (n7);
\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le2] (n27);
\draw (n2) edge[le2] (n28);
\draw (n2) edge[le2] (n32);


\draw (n3) edge[le2] (n7);
\draw (n3) edge[le3] (n12);
\draw (n3) edge[le2] (n13);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);
\draw (n8) edge[le2] (n32);
\draw (n8) edge[le2] (n33);
\draw (n9) edge[le3] (n33);
\draw (n13) edge[le2] (n33);
\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le3] (n32);
\draw (n18) edge[le3] (n33);
\draw (n19) edge[le2] (n33);
\draw (n20) edge[le2] (n32);
\draw (n20) edge[le2] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);
\draw (n23) edge[le2] (n25);
\draw (n23) edge[le2] (n27);
\draw (n23) edge[le2] (n32);
\draw (n24) edge[le2] (n25);
\draw (n24) edge[le2] (n27);

\draw (n25) edge[le2] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le2] (n33);
\draw (n28) edge[le2] (n31);
\draw (n28) edge[le2] (n33);
\draw (n29) edge[le2] (n32);
\draw (n29) edge[le2] (n33);
\draw (n30) edge[le2] (n32);
\draw (n30) edge[le2] (n33);
\draw (n31) edge[le2] (n32);
\draw (n31) edge[le2] (n33);

\end{pgfonlayer}




% strong weak 11 38
%  len: 38 11  set: [(0, 7), (0, 8), (0, 13), (0, 19), (0, 31), (1, 3), (1, 13), (1, 19), (1, 30), (2, 7), (2, 8), (2, 13), (2, 27), (2, 28), (2, 32), (3, 7), (3, 13), (8, 32), (8, 33), (13, 33), (19, 33), (20, 32), (20, 33), (23, 25), (23, 27), (23, 32), (24, 25), (24, 27), (25, 31), (27, 33), (28, 31), (28, 33), (29, 32), (29, 33), (30, 32), (30, 33), (31, 32), (31, 33)] - [(0, 1), (0, 2), (0, 3), (1, 2), (1, 7), (2, 3), (8, 30), (23, 29), (23, 33), (24, 31), (32, 33)]
% lam: 0.6 density : 1.7789473684210524 size: 19
% --- 0.6510589122772217 seconds ---
% {0, 1, 2, 3, 7, 8, 13, 19, 20, 23, 24, 25, 27, 28, 29, 30, 31, 32, 33}




% V(W): 78  E(W): 393
% V(W): 47  E(W): 146
% charikar strong weak 7 40
%  len: 40 7  set: [(0, 1), (0, 3), (0, 7), (0, 8), (0, 13), (0, 19), (0, 31), (1, 7), (1, 19), (1, 30), (2, 3), (2, 7), (2, 8), (2, 13), (2, 27), (2, 28), (2, 32), (3, 7), (3, 13), (8, 32), (8, 33), (13, 33), (19, 33), (23, 25), (23, 27), (23, 29), (23, 32), (23, 33), (24, 25), (24, 31), (25, 31), (27, 33), (28, 31), (28, 33), (29, 33), (30, 32), (30, 33), (31, 32), (31, 33), (32, 33)] - [(0, 2), (1, 2), (1, 3), (1, 13), (8, 30), (24, 27), (29, 32)]
% charikar: lam: 0.6 density : 1.7222222222222223 size: 18
% --- 0.881458044052124 seconds ---
% [0, 1, 2, 3, 7, 8, 13, 19, 23, 24, 25, 27, 28, 29, 30, 31, 32, 33]




% V(W): 78  E(W): 393
% V(W): 47  E(W): 146
% Goldberg  based: strong weak 7 40
%  len: 40 7  set: [(0, 1), (0, 3), (0, 7), (0, 8), (0, 13), (0, 19), (0, 31), (1, 7), (1, 19), (1, 30), (2, 3), (2, 7), (2, 8), (2, 13), (2, 27), (2, 28), (2, 32), (3, 7), (3, 13), (8, 32), (8, 33), (13, 33), (19, 33), (23, 25), (23, 27), (23, 29), (23, 32), (23, 33), (24, 25), (24, 31), (25, 31), (27, 33), (28, 31), (28, 33), (29, 33), (30, 32), (30, 33), (31, 32), (31, 33), (32, 33)] - [(0, 2), (1, 2), (1, 3), (1, 13), (8, 30), (24, 27), (29, 32)]
% goldberg: lam: 0.6 density : 1.7222222222222223 size: 18
% --- 0.4233226776123047 seconds ---
% [0, 1, 2, 3, 32, 33, 7, 8, 13, 19, 23, 24, 25, 27, 28, 29, 30, 31]

==> case-study/r-2-e.tex <==

\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm3] (n17) at (-1.278, -0.60231) {};
\node[lm3] (n18) at (0.51654, 1.9636) {};
\node[lm2] (n19) at (-0.30691, 0.035621) {};
\node[lm3] (n20) at (0.10109, 1.891) {};
\node[lm3] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm2] (n23) at (-0.2767, 1.6423) {};
\node[lm2] (n24) at (-1.5541, 0.77017) {};
\node[lm2] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm2] (n27) at (-0.5343, 0.9102) {};
\node[lm2] (n28) at (-0.16321, 0.83704) {};
\node[lm2] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm2] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};
\begin{pgfonlayer}{background}


\draw (n0) edge[le1] (n2);
\draw (n1) edge[le1] (n2);
\draw (n1) edge[le1] (n3);
\draw (n1) edge[le1] (n13);
\draw (n8) edge[le1] (n30);
\draw (n24) edge[le1] (n27);
\draw (n29) edge[le1] (n32);




\draw (n0) edge[le2] (n1);
\draw (n0) edge[le2] (n3);
\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le3] (n17);
\draw (n0) edge[le2] (n19);
\draw (n0) edge[le3] (n21);
\draw (n0) edge[le2] (n31);
\draw (n1) edge[le2] (n7);
\draw (n1) edge[le3] (n17);
\draw (n1) edge[le2] (n19);
\draw (n1) edge[le3] (n21);
\draw (n1) edge[le2] (n30);
\draw (n2) edge[le2] (n3);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le2] (n7);
\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le2] (n27);
\draw (n2) edge[le2] (n28);
\draw (n2) edge[le2] (n32);
\draw (n3) edge[le2] (n7);
\draw (n3) edge[le3] (n12);
\draw (n3) edge[le2] (n13);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);

\draw (n8) edge[le2] (n32);
\draw (n8) edge[le2] (n33);
\draw (n9) edge[le3] (n33);
\draw (n13) edge[le2] (n33);
\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le3] (n32);
\draw (n18) edge[le3] (n33);
\draw (n19) edge[le2] (n33);
\draw (n20) edge[le3] (n32);
\draw (n20) edge[le3] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);



\draw (n23) edge[le2] (n25);
\draw (n23) edge[le2] (n27);
\draw (n23) edge[le2] (n29);
\draw (n23) edge[le2] (n32);
\draw (n23) edge[le2] (n33);
\draw (n24) edge[le2] (n25);

\draw (n24) edge[le2] (n31);
\draw (n25) edge[le2] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le2] (n33);
\draw (n28) edge[le2] (n31);
\draw (n28) edge[le2] (n33);

\draw (n29) edge[le2] (n33);
\draw (n30) edge[le2] (n32);
\draw (n30) edge[le2] (n33);
\draw (n31) edge[le2] (n32);
\draw (n31) edge[le2] (n33);
\draw (n32) edge[le2] (n33);
\end{pgfonlayer}



==> case-study/r-2-f.tex <==

\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm3] (n17) at (-1.278, -0.60231) {};
\node[lm3] (n18) at (0.51654, 1.9636) {};
\node[lm2] (n19) at (-0.30691, 0.035621) {};
\node[lm3] (n20) at (0.10109, 1.891) {};
\node[lm3] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm2] (n23) at (-0.2767, 1.6423) {};
\node[lm2] (n24) at (-1.5541, 0.77017) {};
\node[lm2] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm2] (n27) at (-0.5343, 0.9102) {};
\node[lm2] (n28) at (-0.16321, 0.83704) {};
\node[lm2] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm2] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};



\begin{pgfonlayer}{background}

\draw (n0) edge[le1] (n2);
\draw (n1) edge[le1] (n2);
\draw (n1) edge[le1] (n3);
\draw (n1) edge[le1] (n13);
\draw (n8) edge[le1] (n30);
\draw (n24) edge[le1] (n27);
\draw (n29) edge[le1] (n32);






\draw (n0) edge[le2] (n1);
\draw (n0) edge[le2] (n3);
\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le3] (n17);
\draw (n0) edge[le2] (n19);
\draw (n0) edge[le3] (n21);
\draw (n0) edge[le2] (n31);
\draw (n1) edge[le2] (n7);
\draw (n1) edge[le3] (n17);
\draw (n1) edge[le2] (n19);
\draw (n1) edge[le3] (n21);
\draw (n1) edge[le2] (n30);
\draw (n2) edge[le2] (n3);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le2] (n7);
\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le2] (n27);
\draw (n2) edge[le2] (n28);
\draw (n2) edge[le2] (n32);
\draw (n3) edge[le2] (n7);
\draw (n3) edge[le3] (n12);
\draw (n3) edge[le2] (n13);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);

\draw (n8) edge[le2] (n32);
\draw (n8) edge[le2] (n33);
\draw (n9) edge[le3] (n33);
\draw (n13) edge[le2] (n33);
\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le3] (n32);
\draw (n18) edge[le3] (n33);
\draw (n19) edge[le2] (n33);
\draw (n20) edge[le3] (n32);
\draw (n20) edge[le3] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);
\draw (n23) edge[le2] (n25);
\draw (n23) edge[le2] (n27);
\draw (n23) edge[le2] (n29);
\draw (n23) edge[le2] (n32);
\draw (n23) edge[le2] (n33);
\draw (n24) edge[le2] (n25);

\draw (n24) edge[le2] (n31);
\draw (n25) edge[le2] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le2] (n33);
\draw (n28) edge[le2] (n31);
\draw (n28) edge[le2] (n33);

\draw (n29) edge[le2] (n33);
\draw (n30) edge[le2] (n32);
\draw (n30) edge[le2] (n33);
\draw (n31) edge[le2] (n32);
\draw (n31) edge[le2] (n33);
\draw (n32) edge[le2] (n33);
\end{pgfonlayer}




==> case-study/r-3-g.tex <==

\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm3] (n17) at (-1.278, -0.60231) {};
\node[lm3] (n18) at (0.51654, 1.9636) {};
\node[lm2] (n19) at (-0.30691, 0.035621) {};
\node[lm3] (n20) at (0.10109, 1.891) {};
\node[lm3] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm3] (n23) at (-0.2767, 1.6423) {};
\node[lm3] (n24) at (-1.5541, 0.77017) {};
\node[lm3] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm3] (n27) at (-0.5343, 0.9102) {};
\node[lm3] (n28) at (-0.16321, 0.83704) {};
\node[lm3] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm3] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};
\begin{pgfonlayer}{background}



\draw (n0) edge[le1] (n1);
\draw (n0) edge[le1] (n2);
\draw (n0) edge[le1] (n3);
\draw (n1) edge[le1] (n2);
\draw (n1) edge[le1] (n3);
\draw (n2) edge[le1] (n3);
\draw (n8) edge[le1] (n30);
\draw (n8) edge[le1] (n32);
\draw (n30) edge[le1] (n32);
\draw (n30) edge[le1] (n33);




\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le3] (n17);
\draw (n0) edge[le2] (n19);
\draw (n0) edge[le3] (n21);
\draw (n0) edge[le3] (n31);
\draw (n1) edge[le2] (n7);
\draw (n1) edge[le2] (n13);
\draw (n1) edge[le3] (n17);
\draw (n1) edge[le2] (n19);
\draw (n1) edge[le3] (n21);
\draw (n1) edge[le2] (n30);
\draw (n2) edge[le2] (n7);
\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le3] (n27);
\draw (n2) edge[le3] (n28);
\draw (n2) edge[le2] (n32);
\draw (n3) edge[le2] (n7);
\draw (n3) edge[le3] (n12);
\draw (n3) edge[le2] (n13);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);


\draw (n8) edge[le2] (n33);
\draw (n9) edge[le3] (n33);
\draw (n13) edge[le2] (n33);
\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le3] (n32);
\draw (n18) edge[le3] (n33);
\draw (n19) edge[le2] (n33);
\draw (n20) edge[le3] (n32);
\draw (n20) edge[le3] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);
\draw (n23) edge[le3] (n25);
\draw (n23) edge[le3] (n27);
\draw (n23) edge[le3] (n29);
\draw (n23) edge[le3] (n32);
\draw (n23) edge[le3] (n33);
\draw (n24) edge[le3] (n25);
\draw (n24) edge[le3] (n27);
\draw (n24) edge[le3] (n31);
\draw (n25) edge[le3] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le3] (n33);
\draw (n28) edge[le3] (n31);
\draw (n28) edge[le3] (n33);
\draw (n29) edge[le3] (n32);
\draw (n29) edge[le3] (n33);

\draw (n31) edge[le3] (n32);
\draw (n31) edge[le3] (n33);
\draw (n32) edge[le2] (n33);
\end{pgfonlayer}




% strong weak 10 18
%  len: 18 10  set: [(0, 7), (0, 8), (0, 13), (0, 19), (1, 7), (1, 13), (1, 19), (1, 30), (2, 7), (2, 8), (2, 13), (2, 32), (3, 7), (3, 13), (8, 33), (13, 33), (19, 33), (32, 33)] - [(0, 1), (0, 2), (0, 3), (1, 2), (1, 3), (2, 3), (8, 30), (8, 32), (30, 32), (30, 33)]
% lam: 0.8 density : 2.2181818181818183 size: 11
% --- 0.11627316474914551 seconds ---
% {0, 1, 2, 3, 32, 33, 7, 8, 13, 19, 30}





% V(W): 78  E(W): 393
% V(W): 47  E(W): 146
% charikar strong weak 7 40
%  len: 40 7  set: [(0, 1), (0, 3), (0, 7), (0, 8), (0, 13), (0, 19), (0, 31), (1, 7), (1, 19), (1, 30), (2, 3), (2, 7), (2, 8), (2, 13), (2, 27), (2, 28), (2, 32), (3, 7), (3, 13), (8, 32), (8, 33), (13, 33), (19, 33), (23, 25), (23, 27), (23, 29), (23, 32), (23, 33), (24, 25), (24, 31), (25, 31), (27, 33), (28, 31), (28, 33), (29, 33), (30, 32), (30, 33), (31, 32), (31, 33), (32, 33)] - [(0, 2), (1, 2), (1, 3), (1, 13), (8, 30), (24, 27), (29, 32)]
% charikar: lam: 0.8 density : 2.1666666666666665 size: 18
% --- 0.12028288841247559 seconds ---
% [0, 1, 2, 3, 7, 8, 13, 19, 23, 24, 25, 27, 28, 29, 30, 31, 32, 33]




% V(W): 78  E(W): 393
% V(W): 47  E(W): 146
% Goldberg  based: strong weak 7 40
%  len: 40 7  set: [(0, 1), (0, 3), (0, 7), (0, 8), (0, 13), (0, 19), (0, 31), (1, 7), (1, 19), (1, 30), (2, 3), (2, 7), (2, 8), (2, 13), (2, 27), (2, 28), (2, 32), (3, 7), (3, 13), (8, 32), (8, 33), (13, 33), (19, 33), (23, 25), (23, 27), (23, 29), (23, 32), (23, 33), (24, 25), (24, 31), (25, 31), (27, 33), (28, 31), (28, 33), (29, 33), (30, 32), (30, 33), (31, 32), (31, 33), (32, 33)] - [(0, 2), (1, 2), (1, 3), (1, 13), (8, 30), (24, 27), (29, 32)]
% goldberg: lam: 0.8 density : 2.1666666666666665 size: 18
% --- 0.16906404495239258 seconds ---
% [0, 1, 2, 3, 32, 33, 7, 8, 13, 19, 23, 24, 25, 27, 28, 29, 30, 31]

==> case-study/r-3-h.tex <==

\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm3] (n17) at (-1.278, -0.60231) {};
\node[lm3] (n18) at (0.51654, 1.9636) {};
\node[lm2] (n19) at (-0.30691, 0.035621) {};
\node[lm3] (n20) at (0.10109, 1.891) {};
\node[lm3] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm2] (n23) at (-0.2767, 1.6423) {};
\node[lm2] (n24) at (-1.5541, 0.77017) {};
\node[lm2] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm2] (n27) at (-0.5343, 0.9102) {};
\node[lm2] (n28) at (-0.16321, 0.83704) {};
\node[lm2] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm2] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};
\begin{pgfonlayer}{background}



\draw (n0) edge[le1] (n2);
\draw (n1) edge[le1] (n2);
\draw (n1) edge[le1] (n3);
\draw (n1) edge[le1] (n13);
\draw (n8) edge[le1] (n30);
\draw (n24) edge[le1] (n27);
\draw (n29) edge[le1] (n32);





\draw (n0) edge[le2] (n1);
\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le2] (n3);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le3] (n17);
\draw (n0) edge[le2] (n19);
\draw (n0) edge[le3] (n21);
\draw (n0) edge[le2] (n31);
\draw (n1) edge[le2] (n7);
\draw (n1) edge[le3] (n17);
\draw (n1) edge[le2] (n19);
\draw (n1) edge[le3] (n21);
\draw (n1) edge[le2] (n30);
\draw (n2) edge[le2] (n3);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le2] (n7);
\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le2] (n27);
\draw (n2) edge[le2] (n28);
\draw (n2) edge[le2] (n32);
\draw (n3) edge[le2] (n7);
\draw (n3) edge[le3] (n12);
\draw (n3) edge[le2] (n13);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);

\draw (n8) edge[le2] (n32);
\draw (n8) edge[le2] (n33);
\draw (n9) edge[le3] (n33);
\draw (n13) edge[le2] (n33);
\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le3] (n32);
\draw (n18) edge[le3] (n33);
\draw (n19) edge[le2] (n33);
\draw (n20) edge[le3] (n32);
\draw (n20) edge[le3] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);
\draw (n23) edge[le2] (n25);
\draw (n23) edge[le2] (n27);
\draw (n23) edge[le2] (n29);
\draw (n23) edge[le2] (n32);
\draw (n23) edge[le2] (n33);
\draw (n24) edge[le2] (n25);

\draw (n24) edge[le2] (n31);
\draw (n25) edge[le2] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le2] (n33);
\draw (n28) edge[le2] (n31);
\draw (n28) edge[le2] (n33);

\draw (n29) edge[le2] (n33);
\draw (n30) edge[le2] (n32);
\draw (n30) edge[le2] (n33);
\draw (n31) edge[le2] (n32);
\draw (n31) edge[le2] (n33);
\draw (n32) edge[le2] (n33);
\end{pgfonlayer}



==> case-study/r-3-i.tex <==

\node[lm2] (n0) at (-0.39521, -0.90369) {};
\node[lm2] (n1) at (-0.1494, -0.63131) {};
\node[lm2] (n2) at (0.089756, -0.058231) {};
\node[lm2] (n3) at (0.32331, -1.0532) {};
\node[lm3] (n4) at (0.023263, -1.9859) {};
\node[lm3] (n5) at (-1.2108, -1.6373) {};
\node[lm3] (n6) at (-0.73841, -1.9544) {};
\node[lm2] (n7) at (0.69671, -1.0172) {};
\node[lm2] (n8) at (0.45414, -0.064462) {};
\node[lm3] (n9) at (1.35, 0.053898) {};
\node[lm3] (n10) at (-0.47034, -1.7978) {};
\node[lm3] (n11) at (-1.6432, -0.89285) {};
\node[lm3] (n12) at (0.52145, -1.7831) {};
\node[lm2] (n13) at (0.59789, -0.39239) {};
\node[lm3] (n14) at (1.15, 1.6278) {};
\node[lm3] (n15) at (1.644, 0.73643) {};
\node[lm3] (n16) at (-1.4464, -2.6101) {};
\node[lm3] (n17) at (-1.278, -0.60231) {};
\node[lm3] (n18) at (0.51654, 1.9636) {};
\node[lm2] (n19) at (-0.30691, 0.035621) {};
\node[lm3] (n20) at (0.10109, 1.891) {};
\node[lm3] (n21) at (-1.1086, -1.0869) {};
\node[lm3] (n22) at (1.4907, 1.075) {};
\node[lm2] (n23) at (-0.2767, 1.6423) {};
\node[lm2] (n24) at (-1.5541, 0.77017) {};
\node[lm2] (n25) at (-1.2836, 1.3377) {};
\node[lm3] (n26) at (1.5531, 1.5267) {};
\node[lm2] (n27) at (-0.5343, 0.9102) {};
\node[lm2] (n28) at (-0.16321, 0.83704) {};
\node[lm2] (n29) at (0.70218, 1.7305) {};
\node[lm2] (n30) at (0.93024, 0.14795) {};
\node[lm2] (n31) at (-0.5944, 0.37166) {};
\node[lm2] (n32) at (0.42538, 0.99008) {};
\node[lm2] (n33) at (0.58393, 0.82341) {};
\begin{pgfonlayer}{background}




\draw (n0) edge[le1] (n2);
\draw (n1) edge[le1] (n2);
\draw (n1) edge[le1] (n3);
\draw (n1) edge[le1] (n13);
\draw (n8) edge[le1] (n30);
\draw (n24) edge[le1] (n27);
\draw (n29) edge[le1] (n32);




\draw (n0) edge[le2] (n1);
\draw (n0) edge[le2] (n3);
\draw (n0) edge[le3] (n4);
\draw (n0) edge[le3] (n5);
\draw (n0) edge[le3] (n6);
\draw (n0) edge[le2] (n7);
\draw (n0) edge[le2] (n8);
\draw (n0) edge[le3] (n10);
\draw (n0) edge[le3] (n11);
\draw (n0) edge[le3] (n12);
\draw (n0) edge[le2] (n13);
\draw (n0) edge[le3] (n17);
\draw (n0) edge[le2] (n19);
\draw (n0) edge[le3] (n21);
\draw (n0) edge[le2] (n31);
\draw (n1) edge[le2] (n7);
\draw (n1) edge[le3] (n17);
\draw (n1) edge[le2] (n19);
\draw (n1) edge[le3] (n21);
\draw (n1) edge[le2] (n30);
\draw (n2) edge[le2] (n3);
\draw (n2) edge[le2] (n13);
\draw (n2) edge[le2] (n7);
\draw (n2) edge[le2] (n8);
\draw (n2) edge[le3] (n9);
\draw (n2) edge[le2] (n27);
\draw (n2) edge[le2] (n28);
\draw (n2) edge[le2] (n32);
\draw (n3) edge[le2] (n7);
\draw (n3) edge[le3] (n12);
\draw (n3) edge[le2] (n13);
\draw (n4) edge[le3] (n6);
\draw (n4) edge[le3] (n10);
\draw (n5) edge[le3] (n6);
\draw (n5) edge[le3] (n10);
\draw (n5) edge[le3] (n16);
\draw (n6) edge[le3] (n16);

\draw (n8) edge[le2] (n32);
\draw (n8) edge[le2] (n33);
\draw (n9) edge[le3] (n33);
\draw (n13) edge[le2] (n33);
\draw (n14) edge[le3] (n32);
\draw (n14) edge[le3] (n33);
\draw (n15) edge[le3] (n32);
\draw (n15) edge[le3] (n33);
\draw (n18) edge[le3] (n32);
\draw (n18) edge[le3] (n33);
\draw (n19) edge[le2] (n33);
\draw (n20) edge[le3] (n32);
\draw (n20) edge[le3] (n33);
\draw (n22) edge[le3] (n32);
\draw (n22) edge[le3] (n33);



\draw (n23) edge[le2] (n25);
\draw (n23) edge[le2] (n27);
\draw (n23) edge[le2] (n29);
\draw (n23) edge[le2] (n32);
\draw (n23) edge[le2] (n33);
\draw (n24) edge[le2] (n25);

\draw (n24) edge[le2] (n31);
\draw (n25) edge[le2] (n31);
\draw (n26) edge[le3] (n29);
\draw (n26) edge[le3] (n33);
\draw (n27) edge[le2] (n33);
\draw (n28) edge[le2] (n31);
\draw (n28) edge[le2] (n33);

\draw (n29) edge[le2] (n33);
\draw (n30) edge[le2] (n32);
\draw (n30) edge[le2] (n33);
\draw (n31) edge[le2] (n32);
\draw (n31) edge[le2] (n33);
\draw (n32) edge[le2] (n33);
\end{pgfonlayer}



==> stats-table-ip-real.tex <==

% \begin{table}[t!]
% \setlength{\tabcolsep}{0pt}
\begin{table*}[t]
% \captionsetup{width=.5\textwidth}
\caption{
Results of the experiments for small-sized real-world datasets. 
Here, $\lambda$ is the parameter in
$\score{\cdot; \lambda}$, columns $\acu$, $\ape$, $\agr$, $\alp$, and $\aip$ represent  \algdenseg, \algdensec, \alggreedyfastest, \alglpstc, and \algip  respectively, columns in $\score{}$ are the discovered scores and columns in $time$ give the computational time in seconds. 
}

\label{tab:ip-result}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name,lam,score-2,score-3,score-1,score-4,score-5,t-2,t-3,t-1,t-4,t-5,s_p-2,s_p-3,s_p-1,s_p-4,s_p-5},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/lam/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/eps/.style={fixed, set thousands separator={\,}, column type=r, column name=$\epsilon$},
    columns/score-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\agr$}, 
    columns/len-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$b$},
    columns/s_p-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\agr$}, 
    columns/w_p-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$w$}, 
    columns/t-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\agr$},
    columns/score-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$\acu$}, 
    columns/len-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$b$},
    columns/s_p-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$\acu$}, 
    columns/w_p-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$w$}, 
    columns/t-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$\acu$},
    columns/score-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ape$}, 
    columns/score-4/.style={fixed, set thousands separator={\,}, column type=r, column name=$\alp$}, 
    columns/score-5/.style={fixed, set thousands separator={\,}, column type=r, column name=$\aip$}, 
    columns/len-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$b$},
    columns/s_p-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ape$}, 
    columns/s_p-4/.style={fixed, set thousands separator={\,}, column type=r, column name=$\alp$}, 
    columns/s_p-5/.style={fixed, set thousands separator={\,}, column type=r, column name=$\aip$}, 
    columns/w_p-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$w$}, 
    columns/t-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ape$},
    columns/t-4/.style={fixed, set thousands separator={\,}, column type=r, column name=$\alp$},
    columns/t-5/.style={fixed, set thousands separator={\,}, column type=r, column name=$\aip$},
    every head row/.style={
		before row={\toprule
		& & 
		\multicolumn{5}{l}{\score{}} &
  		\multicolumn{5}{l}{$time$} &
		\multicolumn{5}{l}{$\abs{E_s}\%$} \\
		\cmidrule(r){3-7}
		\cmidrule(r){8-12}
            \cmidrule(r){13-17}
		},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{ip-real-results.csv}
\end{table*}




==> stats-table-karate.tex <==
\begin{table*}[t]
% \begin{table}[t!]
% \setlength{\tabcolsep}{0pt}
\caption{
Computational statistics from the experiments for  \dtname{Karate} dataset. 
Here, $\lambda$ is the parameter in
$\score{\cdot; \lambda}$, $\score{}$ are the discovered scores,
columns $l$ give the sizes of the discovered subgraph using \alggreedyfastest, \algdenseg, and \algdensec,
columns $\abs{E_s} \%$ give the percentages of {\em strong} edges in the discovered subgraph, columns $t$ give the computational time in seconds, and $g$ indicates whether the greedy algorithm is used or not on finding minimum vertex cover in the wedge graph while running \algdensec and \algdenseg.
}

\label{tab:real-karate-case-study}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name,lam,score-1,len-1,s_p-1,t-1,score-2,len-2,s_p-2,t-2,score-3,len-3,s_p-3,t-3,isgrdy},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/lam/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/score-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\score{}$}, 
    columns/len-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$l$},
    columns/s_p-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E_s} \%$}, 
    columns/w_p-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$w$}, 
    columns/t-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$t$},
    columns/score-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$\score{}$}, 
    columns/len-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$l$},
    columns/s_p-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E_s} \%$}, 
    columns/w_p-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$w$}, 
    columns/t-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$t$},
    columns/score-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$\score{}$}, 
    columns/len-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$l$},
    columns/s_p-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E_s} \%$}, 
    columns/w_p-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$w$}, 
    columns/t-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$t$},
    columns/isgrdy/.style={string type, column type=r, column name=$g$},
    every head row/.style={
		before row={\toprule
		& &
		\multicolumn{4}{l}{\alggreedyfastest} &
		\multicolumn{4}{l}{\algdenseg} &
		\multicolumn{4}{l}{\algdensec} \\
		\cmidrule(r){3-6}
		\cmidrule(r){7-10}
            \cmidrule(r){11-14}
		},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{real-karate.csv}
\end{table*}




==> stats-table-real-small.tex <==
\begin{table*}[t]
% \captionsetup{width=.5\textwidth}
% \begin{table}[t!]
% \setlength{\tabcolsep}{0pt}
\caption{
Characteristics of datasets and computational statistics from the experiments with the real-world datasets using
\alggreedy algorithm.  Here, $\abs{V}$  gives the number of vertices, $\abs{E}$ is the number of edges, $\lambda$ is the weight parameter, $g$ indicates whether greedy algorithm is used or not on finding minimum vertex cover in wedge graph, $\score{}$ gives the discovered score, $size$ is the size of the returned subgraph, $\abs{E_s}$ and $\abs{E_w}$ 
 provide the number of strong and weak edges in the discovered subgraph respectively, $\abs{E_s}\%$ and $\abs{E_w}\%$ give the percentage of strong and weak edges in the discovered subgraph respectively,  and  $time$ gives the computational time in seconds.	
}

\label{tab:real-small}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name,n,m,lam,isgrdy,score,len,s,w,s_p,w_p,t},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Data}},
    columns/n/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{V}$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E}$},
    columns/t/.style={fixed, set thousands separator={\,}, column type=r, column name=$time$},
    columns/lam/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/score/.style={fixed, set thousands separator={\,}, column type=r, column name=$\score{}$}, 
    columns/s_p/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E_s} \%$}, 
    columns/w_p/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E_w} \%$}, 
    columns/len/.style={fixed, set thousands separator={\,}, column type=r, column name=$size$},
    columns/s/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E_s}$},
    columns/w/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E_w}$},
    columns/isgrdy/.style={string type, column type=r, column name=$g$},
    every head row/.style={
		before row={\toprule},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{real.csv}
\end{table*}

==> stats-table-syn-results.tex <==

% \begin{table}[t!]
% \setlength{\tabcolsep}{0pt}
\begin{table*}[t]
% \captionsetup{width=.5\textwidth}
\caption{
Results of the experiments for synthetic datasets. 
Here, $\lambda$ is the parameter in
$\score{\cdot; \lambda}$, columns $\acu$, $\ape$, $\ago$, and $\alp$ represent  \algdenseg, \algdensec, \alggreedyfastest, and \alglpstc respectively, columns in $\score{}$ are the discovered scores, columns in $\abs{E_s} \%$ give the percentages of {\em strong} edges in discovered subgraph, and  columns in time give the computational time in seconds.
}

\label{tab:syn-result}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name,lam,score-2,score-3,score-1,score-4,s_p-2,s_p-3,s_p-1,s_p-4,t-2,t-3,t-1,t-4},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/lam/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/score-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ago$}, 
    columns/len-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ago$},
    columns/s_p-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ago$}, 
    columns/w_p-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ago$}, 
    columns/t-1/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ago$},
    columns/score-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$\acu$}, 
    columns/len-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$b$},
    columns/s_p-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$\acu$}, 
    columns/w_p-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$w$}, 
    columns/t-2/.style={fixed, set thousands separator={\,}, column type=r, column name=$\acu$},
    columns/score-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ape$}, 
    columns/score-4/.style={fixed, set thousands separator={\,}, column type=r, column name=$\alp$}, 
    columns/len-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$b$},
    columns/s_p-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ape$}, 
    columns/s_p-4/.style={fixed, set thousands separator={\,}, column type=r, column name=$\alp$}, 
    columns/w_p-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$w$}, 
    columns/t-3/.style={fixed, set thousands separator={\,}, column type=r, column name=$\ape$},
    columns/t-4/.style={fixed, set thousands separator={\,}, column type=r, column name=$\alp$},
    every head row/.style={
		before row={\toprule
		& &
		\multicolumn{4}{l}{$\score{}$} &
		\multicolumn{4}{l}{$\abs{E_s} \%$} &
		\multicolumn{4}{l}{time} \\
		\cmidrule(r){3-6}
		\cmidrule(r){7-10}
            \cmidrule(r){11-14}
		},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{syn-results.csv}
\end{table*}




==> stats-table-synthetic-data.tex <==

% \begin{table}[t!]
% \setlength{\tabcolsep}{0pt}
\begin{table*}[t]
% \captionsetup{width=.5\textwidth}
\caption{Characteristics of synthetic datasets. Here, $|V^d|$ and $|V^s|$ give an initial number of dense and sparse vertices respectively, $\abs{E}$ is the number of edges, $\abs{C}$ is the true size of the planted clique,
$p_d$, $p_s$, and $p_c$ gives the dense, sparse, and cross edge probabilities, $p_n$ is the noise probability, $d_{true}$ is the ground truth density of the dense component which gives the density of a clique, $\abs{V_z}$ and $\abs{E_z}$ give the number of vertices and edges in the wedge graph.
}

\label{tab:stats-syn-data}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name,n_d,n_s,m,n_w,m_w,clq,spars_pro,cross_pro,noise_pro,true_den},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/n_d/.style={fixed, set thousands separator={\,}, column type=r, column name=$|V^d|$},
    columns/n_s/.style={fixed, set thousands separator={\,}, column type=r, column name=$|V^s|$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E}$},
    columns/clq/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{C}$},
    columns/n_w/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{V_z}$},
    columns/m_w/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E_z}$},    
    columns/true_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{true}$}, 
    columns/den_pro/.style={fixed,set thousands separator={\,},precision=2, column type=r, column name=$p_{d}$},
    columns/spars_pro/.style={fixed,set thousands separator={\,},precision=2, column type=r, column name=$p_{s}$},
    columns/cross_pro/.style={fixed,set thousands separator={\,},precision=2, column type=r, column name=$p_{c}$},
    columns/noise_pro/.style={fixed,set thousands separator={\,},precision=2, column type=r, column name=$p_{n}$},    
    every head row/.style={
		before row={\toprule},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{syn-data.csv}
\end{table*}



